Variation diminishing linear time-invariant systems

This paper studies the variation diminishing property of $k$-positive linear time-invariant (LTI) systems, which map inputs with $k-1$ sign changes to outputs with at most the same variation. We characterize this property for the Toeplitz and Hankel operators of finite-dimensional systems. Our main result is that these operators have a dominant approximation in the form of series or parallel interconnections of $k$ first order positive systems. This is shown by expressing the $k$-positivity of a LTI system as the external positivity (that is, $1$-positivity) of $k$ compound LTI systems. Our characterization generalizes well known properties of externally positive systems ($k=1$) and totally positive systems ($k=\infty$; also known as relaxation systems).

==> sec_compound.tex <==
\section{Compound LTI systems}
\label{sec:compound}
By Proposition~\ref{prop:con_minor_Hankel_Toep}, the variation-diminishing property of Hankel and Toeplitz operators can be verified by showing the positivity of consecutive minors, which are quantities of the type $\det(T_g(t,j))$. We will regard these quantities as impulse responses of so-called {\it compound} systems.
\begin{defn}[Compound systems]
	Let $G(z)$ be an LTI system. Then, for $j \geq 1$ we define  the compound system of order $j$ as the LTI system with impulse response $g_{[j]}(t) := \det(T_g(t,j))$ $t \geq 0$.
\end{defn}
\begin{rem}\label{rem:swap}
	Note that if $t-j\geq 0$, then $T_g(t,j)$ can be transformed into $H_g(t-j+1,j)$ through reversion of the  column/row order, i.e., $\det(T_g(t,j)) = \xi(j)\det(H_g(t-j+1,j))$ where 
	\begin{equation}
	\xi(j) := \begin{cases}
	1 & \text{if } j \mod 4 \leq 1\\
	-1 & \text{else}
	\end{cases}.
	\end{equation}
	 Therefore, an extra definition for $H_g(t,j)$ is generally not required and both cases are treated simultaneously as long as we register $\xi(j)$. Importantly, $2$-positivity can hold simultaneously only for the Hankel and Toeplitz operators of first-order systems.
\end{rem}
Propositions \ref{prop:sr_inf} and \ref{prop:con_minor_Hankel_Toep} lead to the following equivalences. %
\begin{prop} \label{prop:con_minor}
	Let $G(z)$ be a system with $g \in \NF$ and $k \in \mathds{Z}_{>0}$. Then, the following are equivalent:
		\begin{enumerate}[i.]
		\item $\Hank{g}$ is $\tp{k}$. \label{item:Hankel_sr}
		\item \begin{enumerate}
			\item $\forall u \in \linf: \ \vari{u} \leq k-1 \ \Rightarrow \ \vari{\Hank{g} u} \leq \vari{u}$
			\item if $\vari{\Hank{g} u } = \vari{u} \neq 0$ and $u \neq 0$, then the sign of the first non-zero elements in $\Hank{g}u$ and $u$ coincide. 
		\end{enumerate}
		 \label{item:Hankel_vardim} %
		\item $\xi(j) g_{[j]} \mathds{1}_{\mathbb{Z}_{ \geq j}}  \in \NF$ for $2 \leq j \leq k$. \label{item:Hankel_comp}
	\end{enumerate} 
For the Toeplitz operator, let us further assume that the $k-1$-th largest pole is non-zero and $t_0 := \min \{t: g(t) \neq 0\}$. Then, we have the equivalences: 
\begin{enumerate}[I.]
	\item $\Toep{g}$ is $k$-positive. \label{item:Toep_kpos}
	\item $\forall u \in \linf: \ \vari{u} \leq k-1 \ \Rightarrow \ \vari{\Toep{g} u} \leq \vari{u}.$ \label{item:Toep_vardim}
	\item $g_{[j]} \in \NF$ for $1 \leq j \leq k$ and $g_{[j]}(t) > 0$ for $t_0\leq t \leq j-1$ and $1 \leq j \leq k-1$.
\end{enumerate} 
\end{prop}

$k$-positivity of LTI systems can therefore be studied through external positivity of the associated compound LTI systems. It is instructive to consider Proposition~\ref{prop:con_minor} for $k=2$: A function $g \in \NF$ is called \emph{log-concave} if $\supp{g}$ is an interval and 
$$g(t)^2 - g(t-1)g(t+1) = g_{[2]}(t) \geq 0, \;  t \ge 0, $$
this is, the second forward difference of $-\log g$ is nonnegative on $\supp{g}$. In other words, for $k=2$, Proposition~\ref{prop:con_minor} states that a non-FIR LTI system is $2$-positive if and only if its impulse response $g(t)$ is log-concave. It is easy to show that this is also true for FIR systems. 

In statistics, this characterization has been long known for $\tp{2}$ systems under the name of \emph{strongly unimodal distributions} \cite{ibragimov1956composition}. These systems have received considerable attention because of its ability to map unimodal inputs to unimodal outputs. A unimodal signal $u$ has a single  {\it mode} $m \in \mathbb{N}$ such that $u$ is monotonically increasing on $(-\infty, m]$ and monotonically decreasing on $[m,+\infty)$. Equivalently, this means that (\ref{eq:var_diff}) is fulfilled for $\vari{\Delta^{(1)} u} = 0$. In particular, since $\delta(t)$ is unimodal, any $\tp{2}$ kernel must be unimodal and therefore the requirement of $\supp{g}$ being an interval cannot be dropped. 

Similarly, in the Hankel case, it must hold that $g_{[2]}(t) \leq 0, \  t > 0$, meaning that $g$ is log-convex on $\mathds{Z}_{\geq 1}$. Since applying (\ref{eq:Sylvester_id}) to $\det(H_g(\cdot,j+1))$ yields that also $\det(H_g(\cdot,j))$ is log-convex for $1 \leq j \leq k-1$, we obtain the following simplified equivalence. 
\begin{cor}
	\label{cor:consec_minor_hank}
		Let $G(z)$ be a system of order $n$ and $k \leq n$. Then, the following are equivalent:
	\begin{enumerate}[i.]
		\item $\Hank{g}$ is $\tp{k}$. 
		\item $H_g(1,k-1) \succ 0$, $H_g(2,k-1) \succeq 0$ and $\det(H_g(\cdot,k)) \in \NF$. 
		\end{enumerate}
\end{cor} 
Note that this equivalence is an extension of the characterization of totally positive Hankel operators \cite[Theorem~4.4]{pinkus2009totally}.

We next turn to the state-space realization of the compound systems of an  LTI system with realization $(A,b,c)$. 
The definition and properties of the compound matrices and (\ref{eq:Hankel_mat_real}) imply the important property
\begin{equation*}
	\det(H_g(t,j)) s(t-1) = C_{[j]}(\mathcal{O}_j) C_{[j]}(A)^{t-1} C_{[j]} (\mathcal{C}_j)s(t-1), 
	\end{equation*}
this is, the impulse response $\det(H_g(t,j)) s(t-1)$ admits the state-space realization
\begin{equation}
(C_{[j]}(A), C_{[j]} (\mathcal{C}_j), C_{[j]}(\mathcal{O}_j)). \label{eq:ss_compound}
\end{equation}
By Remark~\ref{rem:swap}, it follows that $g_{[j]} \in \NF$ if and only if 
\begin{enumerate}[i.]
	\item $(\xi(j) C_{[j]}(A), C_{[j]} (\mathcal{C}_j), C_{[j]}(\mathcal{O}_j))$ is $1$-positive.
	\item $g_{[j]}(t) \geq 0$ for all $0 \leq t \leq j-1$. 
\end{enumerate}
We note that by Proposition~\ref{prop:con_minor}, the characterization above provides a way of verifying $k$-positivity of a finite dimensional LTI system through verifying external positivity of the state-space model of $j$ compound  systems. While verifying external positivity of any LTI is generally NP-hard \cite{blondel2002presence}, there exist several sufficient tests \cite{anderson1996nonnegative,altafini2016minimal,grussler2012symmetry}. The  test from \cite{grussler2014modified,grussler2019tractable} is particularly tractable through convex programming.
The use of a diagonal state-space representation in the above theorem leads to a characterization of the transfer function $G_{[j]}(z)$ directly in terms of the partial fraction expansion of $G(z)$.
\begin{thm}\label{thm:tpk_poles_coeff}
	Let $G(z) = \sum_{i=1}^{n} \frac{r_i}{z-p_i}$. Then, for $2\leq j \leq n$ it holds that 
	\small \vspace*{-.9 cm}
\begin{multline}
		G_{[j]}(z) = z^{-j} \xi(j) \sum_{v \in \mathcal{I}_{n,j}} \frac{\prod_{i=1}^j r_{v_i} \prod_{(i,j) \in \mathcal{I}_{n,2}} (p_{v_i} - p_{v_j})^2}{z-\prod_{i=1}^j p_{v_i}} \\ +\sum_{i=1}^{j-1} \frac{g_{[j]}(i)}{z^{i}}. \label{eq:compound_tf}
	\end{multline}
	\normalsize
\end{thm}
\vspace*{-.5 cm}These characterizations will be instrumental in the next section. 







==> sec_compound_revised.tex <==
\section{Compound LTI systems}
\label{sec:compound}
Proposition~\ref{prop:con_minor_Hankel_Toep} shows that the variation-diminishing property of LTI systems are studied via the sign of consecutive minors, that is,  quantities of the type $\det(T_g(t,j))$. We will regard these quantities as impulse responses of so-called {\it compound} systems.
\begin{defn}[Compound systems]
	Let $G(z)$ be an LTI system. Then, for $j \geq 1$ we define  the compound system of order $j$ as the LTI system with impulse response $g_{[j]}(t) := \det(T_g(t,j))$ $t \geq 0$.
\end{defn}

A main result of this paper is the following equivalence. %
\begin{thm} \label{prop:con_minor}
	Let $G(z)$ be the transfer function of a causal LTI system with $g \in \NF$ and $k \in \mathds{Z}_{>0}$.  Assume that the $k-1$-th largest pole is non-zero and $t_0 := \min \{t: g(t) \neq 0\}$. Then, we have the equivalences: 
\begin{enumerate}[I.]
	\item $\Toep{g}$ is $k$-positive. \label{item:Toep_kpos}
	\item $\forall u \in \linf: \ \vari{u} \leq k-1 \ \Rightarrow \ \vari{\Toep{g} u} \leq \vari{u}.$ \label{item:Toep_vardim}
	\item $g_{[j]} \in \NF$ for $1 \leq j \leq k$ and $g_{[j]}(t) > 0$ for $t_0\leq t \leq j-1$ and $1 \leq j \leq k-1$.
\end{enumerate} 
\end{thm}

The result shows that $k$-positivity of LTI systems can be studied through external positivity of the associated compound LTI systems. This means that all the results known for positive systems can be leveraged to the characterization of $k$-positive systems. For instance,  $k$-positivity of a finite dimensional LTI system can be verified via the positivity of the state-space model of $j$ compound  systems. While verifying external positivity of any LTI is generally NP-hard \cite{blondel2002presence}, there exist several sufficient tests \cite{anderson1996nonnegative,altafini2016minimal,grussler2012symmetry}. The  test from \cite{grussler2014modified,grussler2019tractable} is particularly tractable through convex programming.


State-space realizations of compound systems are conveniently derived from the Hankel quantities $\det(H_g(t,j))$ rather than from the Toeplitz quantities $\det(T_g(t,j))$ .

We next turn to the state-space realization of the compound systems of an  LTI system with realization $(A,b,c)$. In particular, we observe the important property
\begin{equation*}
	\det(H_g(t,j)) s(t-1) = C_{[j]}(\mathcal{O}_j) C_{[j]}(A)^{t-1} C_{[j]} (\mathcal{C}_j)s(t-1), 
	\end{equation*}
this is, the impulse response $\det(H_g(t,j)) s(t-1)$ admits the state-space realization
\begin{equation}
(C_{[j]}(A), C_{[j]} (\mathcal{C}_j), C_{[j]}(\mathcal{O}_j)). \label{eq:ss_compound}
\end{equation}
By Remark~\ref{rem:swap}, it follows that $g_{[j]} \in \NF$ if and only if 
\begin{enumerate}[i.]
	\item $(\xi(j) C_{[j]}(A), C_{[j]} (\mathcal{C}_j), C_{[j]}(\mathcal{O}_j))$ is $1$-positive.
	\item $g_{[j]}(t) \geq 0$ for all $0 \leq t \leq j-1$. 
\end{enumerate}
The use of a diagonal state-space representation in the above theorem leads to a characterization of the transfer function $G_{[j]}(z)$ directly in terms of the partial fraction expansion of $G(z)$.
\begin{thm}\label{thm:tpk_poles_coeff}
	Let $G(z) = \sum_{i=1}^{n} \frac{r_i}{z-p_i}$. Then, for $2\leq j \leq n$ it holds that 
	\small \vspace*{-.9 cm}
\begin{multline}
		G_{[j]}(z) = z^{-j} \xi(j) \sum_{v \in \mathcal{I}_{n,j}} \frac{\prod_{i=1}^j r_{v_i} \prod_{(i,j) \in \mathcal{I}_{n,2}} (p_{v_i} - p_{v_j})^2}{z-\prod_{i=1}^j p_{v_i}} \\ +\sum_{i=1}^{j-1} \frac{g_{[j]}(i)}{z^{i}}. \label{eq:compound_tf}
	\end{multline}
	\normalsize
\end{thm}
\vspace*{-.5 cm}These characterizations will be instrumental in the next section. 







==> sec_continuous.tex <==
\section{Continuous-time systems}
\label{continuous}
This section extends the results of the previous sections to continuous-time systems. Analogous to discrete time systems, we define the Hankel and Toeplitz operator as %
\begin{subequations}\vspace*{-.7 cm}
	\small
\begin{align*}
	(\Hank{g} u)(t)&:= \int_{-\infty }^{0_{-}} g(t-\tau) u(\tau) d \tau,=  \int_{0_+}^{\infty} g(t+\tau) u(-\tau) d \tau,\\%\label{eq:def_hank_cont}  \\
	(\Toep{g}u)(t) &:= \int_{0}^t g(t-\tau) u(\tau) d\tau. %
	\end{align*}
\end{subequations}
\normalsize
with $g: \mathbb{R} \to \mathbb{R}$ being the impulse response to the causal transfer function $G(s) = \sum_{t=0}^{\infty}g(t)s^{-t}$, i.e., $g(t) = g(t)s(t)$. We will use the convention that the poles of $G(s)$ are sorted by decreasing real part and sub-sorted by decreasing imaginary part. The variation of a signal $u:\mathds{R} \to \mathds{R}$ is defined as 
 \begin{equation}
\vari{u} := \sup_ {\stackrel{n \in \mathbb{Z}_{>0}, x \in \mathds{R}^n}{x_1 < \dots < x_n}} \vari{u(x_1),\dots,u(x_n)}.
\end{equation}
The main idea of characterizing continuous time variation diminishing systems is to discretize the integral operators through finite sums and apply the results from our discrete time discussion. To this end, let us introduce the following definitions \cite{Schoenberg1930vari,karlin1968total}. 
\begin{defn}\label{def:tpk_cont}
	Let $G(s)$ be a causal, asymptotically stable system and \begin{equation}
	K_g(t,\tau) := \begin{pmatrix}
	g(t_1 - \tau_1) & \cdots & g(t_1-\tau_k)\\
	\vdots       &             & \vdots   \\
	g(t_k - \tau_1) & \cdots   & g(t_k-\tau_k)
	\end{pmatrix}
	\end{equation}
		where $t,\tau \in \Delta^k := \{x \in \mathds{R}^k: 0 \leq x_1 < \dots < x_k\}$ and $k \in \mathbb{Z}_{>0}$. Then, $\Toep{g}$ is $\tp{k}$, if $K_g(t,\tau)$ is $\tp{k}$ for all $t,\tau \in \Delta^k$. Analogously, we define this property for $\Hank{g}$ with $K_g(t,-\tau)$.
\end{defn}Indeed, if $(\Hank{g}^{h,N} u)(t) := h \sum_{i=1}^N g(t+\tau_i) u(-\tau_i)$
with $h > 0$, $\tau_i = i h$, then for sufficiently large $N$ and small $h$ it holds that $\vari{\Hank{g}^{h,N}u} = \vari{\Hank{g}u}$. Further, there exist $t_1 < \dots < t_N$ such that $\vari{\hat{y}} = \vari{\Hank{g}u}$ with
\begin{equation*}
\hat{y} := \begin{pmatrix}
g(t_1 + \tau_1) & \cdots & g(t_1+\tau_N)\\
\vdots       &             & \vdots   \\
g(t_N + \tau_1) & \cdots   & g(t_N+\tau_N)
\end{pmatrix} \begin{pmatrix}
u(-\tau_1)\\
\vdots \\
u(-\tau_N)
\end{pmatrix},
\end{equation*}
meaning that if $\Hank{g}$ is $\tp{k}$, then also the mapping above is $\tp{k}$. More generally, by choosing $t_i$ and $\tau_i$ such that \vspace*{-.9 cm}
\small
\begin{equation*}
K_g(t,\tau) = T_{g_h}(t,j) = \begin{pmatrix}
g(th) & \cdots & g((t-j+1)h)\\
\vdots       &             & \vdots   \\
g((t+j-1)h) & \cdots   & g(th)
\end{pmatrix}
\end{equation*} \normalfont where $G_h(z) = \sum_{i= 1}^n \frac{r_i}{z-e^{p_ih}}$, we get the following analogue to Theorem~\ref{thm:tpk_poles_coeff} as a consequence of our discrete analysis. 
\begin{prop}
	Let $G(s) = \sum_{i= 1}^n \frac{r_i}{s-p_i}$, $h >0$ and $g_h(t) := g(th)$. Then,\vspace*{-.2 cm}
		\begin{enumerate}
		\item if $\Toep{g}$ is $\tp{k}$ it holds that $\Toep{g_h}$ is $\tp{k}$, $(-1)^{i+1} r_i >0$ for $1\leq i\leq k$ and $p_1,\dots,p_k \in \mathbb{R}$.  
		\item if $\Hank{g}$ is $\tp{k}$ it holds that $\Hank{g_h}$ is $\tp{k}$, $r_1,\dots,r_k > 0$ and $p_1,\dots,p_k \in \mathbb{R}$.  
	\end{enumerate}
\end{prop}
Furthermore, it is easy to show that if $\Hank{g}$ is $\tp{k}$, then 
\begin{align*}
H^\ast_g(t,j) &:= \begin{pmatrix}
g(t)& \dfrac{d}{dt} g(t) & \cdots & \dfrac{d^{j-1}}{dt^{j-1}}g(t)\\
\dfrac{d}{dt} g(t) & \dfrac{d^2}{dt^2}g(t) & \cdots & \dfrac{d^{j}}{dt^{j}}g(t)\\
\vdots       &     \vdots    &     & \vdots   \\
\dfrac{d^{j-1}}{dt^{j-1}}g(t) & \dfrac{d^{j}}{dt^{j}}g(t) & \cdots   & \dfrac{d^{2j-2}}{dt^{2j-2}} g(t)
\end{pmatrix}.
\end{align*}
fulfils $\det(H^\ast_g(t,j)) \geq 0$. Analogous, for $\tp{k}$ $\Toep{g}$ we get that $\det(T^\ast_g(t,j)) \geq 0$ for $1 \leq j  \leq k$ with
\begin{align*}
T^\ast_g(t,j) = \begin{pmatrix}
\dfrac{d^{j-1}}{dt^{j-1}}g(t) & \cdots & \dfrac{d}{dt} g(t) & g(t) \\
\dfrac{d^{j}}{dt^{j}}g(t) & \cdots & \dfrac{d^2}{dt^2}g(t) & \dfrac{d}{dt} g(t)\\
\vdots       &      &     \vdots    & \vdots   \\
\dfrac{d^{2j-2}}{dt^{2j-2}} g(t)  &\cdots & \dfrac{d^{j}}{dt^{j}}g(t)  & \dfrac{d^{j-1}}{dt^{j-1}}g(t)
\end{pmatrix}.
\end{align*}
Converse results of this observation as in Proposition \ref{prop:con_minor} and Corollary \ref{cor:consec_minor_hank} can be proven, where the compound systems are defined by $g_{[j]} := \det(T_g^\ast(t,j))$. In particular, the case with $g_{[j]} \in \mathcal{F}_{>0}$ for $1 \leq j \leq k-1$ has been discussed in \cite{karlin1968total}. For the Hankel operator, this condition can be relaxed to non-strictness: analogues to \cite{fallat2017total}, Hankel strictly $\tp{k}$ systems lie densely within set of Hankel $\tp{k}$ systems. 



Further, for a system $G(s)$ with realization $(A,b,c)$ it holds as in the discrete-time case that 
\begin{equation*}
\det(H_g^\ast(t,j)) = {C}_{[j]}(\mathcal{O}_j) {C}_{[j]}(e^{At}) {C}_{[j]}(\mathcal{C}_j).
\end{equation*}
Since ${C}_{[j]}(e^{At}) = e^{\log(C_{[j]}(e^A))t}$, $\det(H_g^\ast(t,j))$, $t \geq 0$, has a realization $(\log(C_{[j]}(e^A)),{C}_{[j]}(\mathcal{C}_j),{C}_{[j]}(\mathcal{O}_j)).$ Theorem~\ref{thm:decomp_tpk} can then be easily transferred as follows.  
\begin{thm}\label{thm:decomp_tpk_cont}
	Let $G(s) = \sum_{i=1}^{n} \frac{r_i}{s-p_i}$ and $k \leq n$.
	\vspace*{-.2 cm}
	\begin{enumerate}
		\item If $\Toep{g}$ is $\tp{k}$, then 
		$G(s) = \frac{1}{s-p_1}  G_r(s)$, where $\Toep{g_r} \text{ is } \tp{k-1}$
	   and all real zeros are smaller than $p_k$. 
		\item 	If $\Hank{g}$ is $\tp{k}$, then $G(s) = \frac{r_{1}}{s-p_1} + G_r(s)$, where $r_{1} > 0$ $\Hank{g_r}$ is  $\tp{k-1}$.
	\end{enumerate}
\end{thm}
Note the slight deviation in the Toeplitz case, which is a result of the absence of FIR dynamics as the following result on Toeplitz $\tp{2}$ systems reveals.
 \begin{lem} \label{lem:no_d}
 	Let $G(s)$ be an LTI system with $\Toep{g}$ being $\tp{2}$. Then, $G(s)$ is strictly proper.
 \end{lem}
Thus, by Theorem~\ref{thm:decomp_tpk_cont}, we recover the results from \cite{Aissen1952generating,fekete1912uber,karlin1968total,willems1976realization} for total positivity.

\begin{prop}\label{prop:toep_inf_pos_cont}
Let $G(s) = \sum_{i=1}^{n} \frac{r_i}{s+p_i}$. \vspace*{-.2 cm}
\begin{enumerate}[i)]
	\item $\Toep{g}$ is totally positive if and only if
	$G(s) =  \frac{r}{\prod_{i=1}^n (s+p_i)}$
	where $r_i > 0$ and $p_i \in \mathds{R}$. 
	\item $\Hank{g}$ is totally positive if and only if $
	G(s) = \sum_{i=1}^{n} \frac{r_i}{s+p_i}$
where $r_i > 0$ and $p_i \in \mathds{R}$.
\end{enumerate}
\end{prop}


==> sec_examples.tex <==
\section{Examples}
\label{sec:app}
In this section, we will discuss several examples of $\tp{k}$ systems, which we use to illustrate our theory as well as to point out future directions and relationships to recent related work. 


\subsection{Neuronal networks}
Physiological neuronal networks are often modelled as a parallel interconnection of externally positive subsystems of type
\begin{equation*}
G_a(z) = \frac{k_1}{z-p_1}, \quad G_b(z)= \frac{k_2}{z-p_2} - \frac{k_3}{z-p_3},
\end{equation*}
followed by a non-decreasing activation function such as the sigmoid function. \textcolor{blue}{Rodolphe: Can you add a reference and perhaps background on ion channels/fading memory?} We will now see that such a systems can have various degrees of local extrema diminishment from past input to future output. 

To see this, we first note that non-decreasing non-linearities are local extrema diminishing by the chain rule. Further, Hankel variation diminishing systems are due to linearity also local extrema diminishing, which is why we only need to analyse the variation diminishing property of the linear system part. If all subsystems are of type $G_a(z)$, it follows from Proposition~\ref{prop:toep_inf_pos} that the neuronal network is Hankel totally \ovd. In many other cases, however, the network can be at most \ovd{k} for finite $k$ by Theorem~\ref{prop:con_minor} and \ref{thm:decomp_tpk}.

For example, let $G(z) = G_a(z) + G_b(z)$ with all $k_i,p_i > 0$, $p_i$ distinct, $k_2 \geq k_3$ and $p_2 > p_3.$ Then, $G(z)$ is Hankel $\tp{1}$ as a sum of externally positive systems, but at most $\tp{2}$ by Theorem~\ref{thm:decomp_tpk}. To decide the latter, we need to check by Theorem~\ref{prop:con_minor} and \ref{thm:tpk_poles_coeff} if
\begin{equation*}
G_{[2]}(z) = \frac{r_1r_2 (p_1-p_2)^2}{z-p_1p_2}- \frac{r_1r_3 (p_1-p_3)^2}{z-p_1p_3} -  \frac{r_2 r_3 (p_2-p_3)^2}{z-p_2p_3}
\end{equation*}
\normalsize
is externally positive. It is easy to see that this is the case if and only if $p_1p_2 \geq p_1p_3$ and $r_1 r_2 \geq r_1r_3 + r_2 r_3$. 

As the role of the Hankel \ovd{k} property seems to be neglected in the analysis of such networks, our work can be considered a first step towards this novel understanding. 










\subsection{Heavy-ball method}
The so-called heavy-ball method for (convex) optimization was designed by Polyak to damp the possibly high number of local extrema in the iterates of the well-known gradient descent approach \cite{polyak19641methods,ghadimi2015global}. For a convex function $f: \mathbb{R} \to \mathbb{R}$, the iterates $x(k)$ of this method are given by the closed-loop system
\begin{align*}
x({k+1}) &= x(k) + \alpha u(k) + \beta (x(k) - x({k-1}))\\
y(k) &= \left . \frac{d}{dx}f(x) \right |_{x = x_k} \\
u(k) &= -y
\end{align*}
for constant $\alpha,\beta > 0$. Since the linear system from $u$ to $x$ reads $G(z) = \frac{\alpha z}{(z-1) (z - \beta)}$, it is Toeplitz totally \ovd{} by Proposition~\ref{prop:toep_inf_pos}. Further, as the derivatives of convex functions are non-decreasing \cite{Boyd2004}, it follows as above that the entire open loop system from $u$ to $y$ is local extrema diminishing. 

To also analysis the closed-loop system, let us assume that $f$ is quadratic. Then, $y(k) = ax - b$ with $a > 0$, i.e., $y$ is the response of a linear closed-loop system to a step with height $b$. It is easy to show that the closed-loop system is Toeplitz totally \ovd{} if and only if $\beta \geq (\sqrt{a \alpha}+1)^2$. This observation verifies the intuition that the required amount of momentum (damping) for variation diminishment scales with the the gain of the gradient, which in the optimization literature is associated with the Lipschitz constant of the gradient \cite{ghadimi2015global}. Then, choosing $x(0) = 0$ results in iterates without local extrema. In particular, local extrema from noisy gradients (which may be modelled as time-varying $b$) can be diminished independently of the noise distribution. Since suggested choices for $\alpha$ and $\beta$ \cite{ghadimi2015global,polyak19641methods} do not necessarily result in closed-loop total \ovd{}, an investigation of the effects of Toeplitz $\tp{k}$ designs to convergence rates and robustness seems highly desirable. 

This application demonstrates the importance of variation diminishing theory in optimization and motivates the extension of our theory to non-linear negative feedback interconnections. Note that in case of multi-dimensional iterates, the algorithm as well as our analysis applies component-wise. Further, since $G(z)$ permits a minimal realization $(A,b,c)$ with totally positive $A$, it becomes evident how our analysis complements the study of autonomous $k$-positive systems \cite{weiss2019generalization,margaliot2018revisiting}. 


\subsection{Monotone Cyclic Feedback Systems}
\emph{Monotone cyclic feedback systems} are autonomous systems with the properties 
\begin{align*}
& x_i(k+1) = f_i(x_i(k),x_{i-1}(k)), \; i = 1,\dots,n, \; x_0 := x_n, \\
& \delta_i \frac{\partial f_i(x_i(k),x_{i-1}(k))}{\partial x_{i-1}(k)} > 0,
\end{align*}
where $|\delta_i| = 1$ \cite{MalletParet1990}. In other words, these systems are closed-loop systems, whose open loop dynamics consists of the serial interconnection of non-linear first order systems, where each non-linearity $f_i$ is increasing in $x_{i-1}$. System of this type occur frequently in biology, e.g., if each first order system is the firing-rate model of a neuron, then $f_i(x_i,x_{i-1}) = p_i x_i + b_i s(x_{i-1})$, where $p_i, b_i > 0$ and $s$ is an increasing activation function. 

While a Poincar{\'e}-Bendixon theorem for these system has been known since~\cite{MalletParet1990}, its simplified Lyapunov theory based on sign-changes has only been noted recently \cite{avraham2020dynamical}. The present work opens up the complementary route towards an open loop analysis, which as noted in previous examples invokes Toeplitz totally positivity. As in the discussion of the heavy-ball methods, this path would make it easy to incorporate exogenous inputs such as references and disturbance signals as well as to extend the open-loop dynamics to Toeplitz $k$-positivity. 

==> sec_extensions.tex <==
\section{Repeated Poles}
\label{sec:ext}
The results in the previous sections were stated for LTI systems with simple poles. 
The restriction simplified the exposition, because the dominant dynamics of $G_{[j]}$ take a more complicated form in the general case. For the Hankel operator, however, the additional effort is minimal. To see this, let $G(z)$ have $l$ distinct poles with highest multiplicity $m_j$, $1 \leq j \leq l$, this is,  
\begin{align*}
G(z) = \sum_{a=1}^{l} \sum_{b=1}^{m_a} \frac{r_{ba}}{(z-p_a)^b}.
\end{align*} 
Then, external positivity requires that $r_{1m_1} > 0$ and $p_1 \geq 0$. Assuming that $m_1 > 1$ and $p_1 > 0$, it follows then that the dominant dynamics of $g_{[2]}$ are provided by $G_1(z) := \frac{r_{1m_1}}{(z-p_1)^{m_1}}$. Since $g_1$ not log-convex on any interval, $\Hank{g}$ cannot be $\tp{2}$. Further, it is easy to see that the only FIR system that is Hankel $\tp{2}$ is a first order system. 
Similarly, assuming that $m_1 = \dots = m_{k-2} = 1$ and $m_{k-1} > 1$, it follows by (\ref{eq:ss_compound}) that the dominant dynamics of $G_{[k-1]}$ have a multiple pole in $\prod_{i=1}^{k-1}p_i$. However, since $g_{[k-1]}$ also needs to be log-convex on $\mathds{Z}_{\geq k-1}$, $\Hank{g}$ cannot be $k$-positive then.
\begin{prop}
	Let $G(z) = \sum_{a=1}^{l} \sum_{b=1}^{m_a} \frac{r_{ba}}{(z-p_a)^b}$ be such that $\Hank{g}$ is $k$-positive. Then, $m_1 = \dots = m_{k-1} = 1$.
\end{prop}








==> sec_k_pos_revRS.tex <==
\section{Dominant decompositions of $k$-positive systems}
\label{sec:k_pos}

The characterization in the previous section has interesting implications about the poles and zeros of variation-diminishing systems. This can be regarded as a consequence of the Perron-Frobenius theorem \cite{horn2012matrix} applied to the positivity of the compound systems.

\subsection{Positive and totally  positive systems}

We begin this section by recalling well-known pole-zero characterizations of externally positive (this is, $\tp{1}$)  and totally positive (this is, $\tp{\infty}$) systems.


A characterization of %
$\Toep{g}$ being $\tp{\infty}$ in terms of its poles and zeros goes back (at least) to \cite{Aissen1952generating}. Similar results for the continuous-time Hankel operator can also be found in \cite{karlin1968total}. We supplement these results for the discrete time Hankel case. 
\begin{prop}\label{prop:toep_inf_pos}
	Let $G(z)$ be strictly proper. Then, 

\begin{enumerate}[i)]
	\item $\Toep{g}$ is totally positive if and only if
	$G(z) =  \prod_{i=1}^n \frac{r_i z+\alpha_i}{z-p_i}$
	$\alpha_i, r_i, p_i \geq 0$, i.e., it is the serial interconnection of first order positive filters with negative zeros.
	\item $\Hank{g}$ is totally positive if and only if $G(z) = \sum_{i=1}^{n} \frac{r_i}{z-p_i}$,
	where $r_i , p_i \geq 0$, i.e., it is the parallel interconnection of first order externally positive filters.
\end{enumerate}
\end{prop}
Note that the negative zeros requirement in the Toeplitz case can be seen as a consequence of the positive poles by using  the following key property \cite{karlin1968total}.
\begin{lem}\label{eq:lem_inv}
	Let $G(z)$ have relative degree $n-m$. Then, $\Toep{g}$ is $\tp{\infty}$ if and only if $\Toep{\tilde{g}}$ with $\tilde{G}(z) :=\frac{(-z)^{m-n}}{G(-z)}$ is totally positive. 
\end{lem}












\subsection{Poles and zeros of $k$-positive systems}


The following results generalizes Proposition~\ref{prop:dominantpole}  ($k=1$) and Proposition~\ref{prop:toep_inf_pos} ($k=+\infty$) to  $k$-positive systems with $k$ arbitrary and represent our main contributions.

\begin{thm}\label{cor:tpk_coeff}
	Let $G(z) = \sum_{i=1}^{n} \frac{r_i}{z-p_i}$, let $k \in \mathbb{Z}_{>0}$ and $m := \min\{k,n\}$. Then,
	\begin{enumerate}
		\item if $\Toep{g}$ is $\tp{k}$ it holds that $(-1)^{i+1} r_i >0$ for $1\leq i\leq m$ and $p_1,\dots,p_m \geq 0$.
		\item if $\Hank{g}$ is $\tp{k}$ it holds that $r_1,\dots,r_m > 0$ and $p_1,\dots,p_m \geq 0$.
	\end{enumerate}
\end{thm}
\begin{pf}
The proof follows from Theorem~\ref{thm:tpk_poles_coeff} and the application of Proposition~\ref{prop:dominantpole} to the first order dominant dynamics of $G_{[j]}$ as well as Remark~\ref{rem:swap} for the Hankel case. 	
\end{pf}




\begin{thm}\label{thm:decomp_tpk}
	Let $G(z) =  \sum_{i=1}^{n} \frac{r_i}{z-p_i}$ and $k \leq n$.  
\begin{enumerate}
	\item If $\Toep{g}$ is $\tp{k}$, then $
	G(z) = \frac{z}{z-p_1}  G_r(z)$, where $\Toep{g_r} \text{ is } \tp{k-1}$
	and all real zeros are smaller than $p_{\min\{k,n\}}$. 
	\item 	If $\Hank{g}$ is $\tp{k}$, then $G(z) = \frac{r_{1}}{z-p_1} + G_r(z)$, where $\Hank{g_r} \text{ is } \tp{k-1}$ with $r_{1} > 0$.
\end{enumerate}

\end{thm}
A repeated application of Theorem~\ref{thm:decomp_tpk} shows that $k$-positive systems possess a $k$-th order dominant approximation that is totally positive with respect to their operators. Again, that result is well-known for $1$-positive systems and for totally positive systems but appears novel for other values of $k$. Unfortunately, our result does not provide a full characterization of $k$-positivity, but only necessary conditions. The example in Figure~\ref{fig:notsuff} illustrates a second-order system that is not Toeplitz $\tp{2}$, but has a dominant first-order approximation. A full characterization for finite $k$ can also not be expected given the NP-hardness of the case $k=1$.  
\begin{figure}
	\centering
\begin{tikzpicture}
\begin{groupplot}[group style={group name=my plots, group size=1 by 1,vertical sep=2.2 cm}, height = 3.5 cm, width = 9 cm]
\nextgroupplot[
xlabel= {$t$},
ylabel = {$g(t)$},
xmin = 0,
xmax = 30,
scaled ticks=false, 
tick label style={/pgf/number format/fixed}]
\addplot[ycomb, color = FigColor1] file{ex_decomp.txt};
\end{groupplot}
\end{tikzpicture}
\caption{$g := g_1 \ast g_2$ with $g_1(t) = 0.9^{t-1} s(t-1)$ and $g_2(t) = 0.8^{t-1}(1+cos(\frac{\pi(t-1)}{2}))s(t-1)$ is not unimodal, but $G(z) = \frac{1}{z-0.9} G_2(z)$ with $\Toep{g_2}$ being $\tp{1}$.\label{fig:notsuff}}
\end{figure}
Finally, note that the smoothness of Hankel $k$-positive systems can also be seen in the forward differences of their impulse responses.
 \begin{lem}
	\label{lem:diff_Hank}
	Let $G(z) = \sum_{i = 1}^n \frac{r_i}{z-p_i}$ be such that $g \in \NF \cap \linf$ and $\Hank{-\Delta^{(1)} g}$ is $\tp{k}$. Then, $\Hank{g}$ is $\tp{k}$.
	Conversely, if all $k_i > 0$ and $p_i \geq 0$, this is, $\Hank{g}$ is totally positive, then also $\Hank{-\Delta^{(1)} g}$ is totally positive.  
\end{lem} 




















==> sec_mot_revRS.tex <==
\section{The variation diminishing property}
\label{sec:vardim}
\subsection{Variation diminishing systems}
 For a function $g: \mathds{Z} \to \mathbb{R}$ its \emph{variation (number of sign changes)} is defined as
 \begin{equation}
 \vari{g} := \sup_ {\stackrel{n \in \mathbb{Z}_{>0}, x \in \mathds{Z}^n}{x_1 < \dots < x_n}} \vari{g(x_1),\dots,g(x_n)}.
 \end{equation}
 where
$\vari{x} := \sum_{i \geq 1} \mathbb{1}_{\mathbb{R}_{< 0}}(\tilde{x}_i \tilde{x}_{i+1})$ is the \emph{variation} for $x \in \mathbb{R}^n$ with  $\tilde{x}$ resulting from deleting all zero entries in $x$ and $\vari{0} := -1$. Investigations of linear \emph{variation diminishing} mappings $y = Xu$, i.e., $\vari{y} \leq \vari{u}$ for all $u$ with $\vari{u}\leq k \in \mathds{Z}_{\geq 0}$ date back from the investigation of power series with real zeros \cite{fekete1912uber} to applications in interpolation theory \cite{Schoenberg1951polya,karlin1968total}, vibrational systems \cite{gantmacher1950oszillationsmatrizen} and computer vision \cite{lindeberg1990scale}. $X$ may therefore represent finite dimensional matrices as in \cite{Schoenberg1930vari,karlin1968total} as well as infinite dimensional operators such as the Toeplitz and Hankel operator \cite{karlin1968total,Schoenberg1951polya,Samworth2017,ibragimov1956composition}. 

The goal of this paper is to provide a characterization of variation diminishing finite-dimensional LTI systems with input $u$ and output $y$. We consider both, their Hankel and Toeplitz operators: 
\begin{subequations}
	\begin{align}
	y &= \Toep{g}u: &\vari{\Toep{g}u} &\leq \vari{u} \leq k-1, \label{eq:toep_dem} \\
	y &= \Hank{g}u: &\vari{\Hank{g}u} &\leq  \vari{u} \leq k-1 \label{eq:hank_dem},
	\end{align}
\end{subequations}
The characterization  of $k$-positive systems provides any intermediate between the coarsest variation-diminishing property of positive systems ($k=1$) and the finest variation diminishing property ($k= \infty$).  %

It should be noted that due to linearity, the variation-diminishing property of LTI systems does not only apply variation of the input-output signals but also to any of their finite differences. As such, linear variation diminishing systems also diminish local extrema, inflections points, etc., this is, for all $s \geq 1$ and $u$ it holds that
\begin{align}
\vari{\Delta^{(s)}u} \leq k-1 \ \Longrightarrow \  \vari{\Delta^{(s)}y} \leq \vari{\Delta^{(s)}u}. \label{eq:var_diff} %
\end{align}
These systems, therefore,  posses a low-pass characteristic and the maximal choosable $k$ determines a a degree of smoothening. The simplest example of a variation diminishing system is an integrator. As first order filters are damped versions of an integrator, the same can be expected for them as discussed next.







\begin{example}
	\label{ex:first_order}
	The impulse response of a first order system
\begin{align*}
g (t) = {r p^{t-1}} s(t-1), \ p >0, \ r \in \mathbb{R}
\end{align*}
with transfer function $G (z) = \frac{r}{z-p}, \ |z| > p$ %
has Hankel and Toeplitz operators
\begin{subequations}
\begin{align}
(\Hank{g}{u})(t) &= \alpha r p^{t-1}, \ t \geq 1, \; \alpha:= \sum_{\tau = -\infty}^{-1} p^{-\tau} {u}(\tau) \label{eq:Hank_first}\\
(\Toep{g}{u})(t) &= r p^{t-1} \sum_{\tau = 1}^{t} p^{-\tau} {u}(\tau), \; t \geq 0 \label{eq:Toep_first}
\end{align}
\end{subequations}
The Hankel operator is a decaying exponential multiplied by a scalar. Hence it has no variation, regardless of the variation of the input. 
The Toeplitz operator maps  nonnegative/monotone inputs  to nonnegative/monotone outputs because the first-order filter  is positive. Thus, only a sign-change in $u$ can cause the sum in (\ref{eq:Toep_first}) to change sign for $t \geq 0$. However, since the summand has the same variation as $u$ and summation (integrator) cannot increase the variation, $\vari{\Toep{g}{u}} \leq \vari{u}$ for all $u$. 
\end{example}
For general LTI systems, we will study the variation diminishing property of the operators through the variation diminishing properties of matrices, that correspond to  the finite dimensional truncations $\Hank{g}^n u$ and $\Toep{g}u$. The correspondence is formalized as follows \cite{Schoenberg1951polya}.
\begin{prop}\label{prop:op_seq}
	Let $g \in \mathbb{R}^{\mathds{Z}}$ and $k \in \mathbb{Z}_{\geq 1}$. Then, the following are equivalent:
	\begin{enumerate}[i)]
		\item $\vari{\Hank{g}u}  \leq \vari{u} $ for all $u\in \mathbb{R}^{\mathds{Z}}$ such that $\Hank{g}u \in \linf$ and $\vari{u} \leq k-1$ \label{item:op_var_dim}
		\item $\forall n \in \mathds{Z}_{\geq 0}: \vari{\Hank{g}^nu}  \leq \vari{u}$ for all $u\in \mathbb{R}^{\mathds{Z}}$ such that $\Hank{g}u \in \linf$ and $\vari{u} \leq k-1$. \label{item:sequence_var_dim}
	\end{enumerate}
	Analogous results hold for $\Toep{g}u$.
\end{prop}










==> sec_vardim_new_revRS.tex <==


\subsection{Variation diminishing matrices}
The theory of variation diminishing matrices is a classical subject, for instance extensively studied in the monograph \cite{karlin1968total}. Variation diminishing properties of a matrix $X \in \Rmn$ are studied via the sign-definiteness of the compound matrices $C_r(X)$, whose $(i,j)-th$ entry is defined by $\det(X_{(I,J)})$, where $I$ is the $i-th$ and $J$ is the $j-th$ element in $\mathcal{I}_{n,r}$ and $\mathcal{I}_{m,r}$, respectively. 
For example, if $X \in \mathbb{R}^{3 \times 3}$, then $C_{[2]}(X)$ reads
\begin{align*}
\begin{pmatrix}
\det(X_{\{1,2 \},\{1,2 \}}) & \det(X_{\{1,2 \},\{1,3\}}) & \det(X_{\{1,2 \},\{2,3\}})\\
\det(X_{\{1,3 \},\{1,2 \}}) & \det(X_{\{1,3 \},\{1,3\}}) & \det(X_{\{1,3 \},\{2,3\}})\\
\det(X_{\{2,3 \},\{1,2 \}}) & \det(X_{\{2,3 \},\{1,3\}}) & \det(X_{\{2,3 \},\{2,3\}})\\
\end{pmatrix}.
\end{align*}
made of all $r$-minors. 
By the \emph{extended Cauchy-Binet formula} \cite{karlin1968total} with $X \in \mathbb{R}^{n \times p}$ and $Y \in \mathbb{R}^{p \times m}$
\begin{equation}
\det((XY)_{I,J}) = \sum_{K \in \mathcal{I}_{p,r}} \det(X_{I,K}) \det(Y_{K,J}), \label{eq:CB}
\end{equation}
where $I \in \mathcal{I}_{n,r}$, $J \in \mathcal{J}_{m,r}$ and $r \leq p$, it easy to verify the following well-known properties \cite[Chapter~6]{fiedler2008special}. 
\begin{lem}\label{lem:compound_mat}
	Let $X \in \mathbb{R}^{n \times p}$, $Y \in \mathbb{R}^{p \times m}$ and $r \in \mathds{Z}_{\geq 1}$.
	\begin{enumerate}[i)]
		\item $C_{[r]}(XY) = C_{[r]}(X)C_{[r]}(Y)$.
		\item $\sigma(C_{[r]}(X)) = \{\prod_{i \in I} \lambda_i(X): I \in \mathcal{I}_{n,r} \}$.
		\item If $X \succeq 0$, then $C_{[r]}(X) \succeq 0$.
	\end{enumerate} 
\end{lem}

\begin{defn}[Sign-consistency and -regularity]
\label{def:sc}
	A matrix is called \emph{ $k$-sign consistent}  if all its  minors of order $k$ have the same sign. The property is {\it strict} if none of those minors is zero. 
The same matrix  is called \emph{(strictly) $k$-sign regular}, if it is (strictly) $j$-sign consistent for all $1 \leq j \leq k$. It is called {\emph (strictly)  $k$-positive} if the sign of minors is the same for all $1 \leq j \leq k$.
\end{defn}

The relationship between the variation diminishing property and the above definitions is provided by combining the results \cite[Theorem~5.1.1.4, Theorem~5.1.1.5,Theorem~5.2.2.4,]{karlin1968total} as follows.
\begin{prop} \label{prop:SR}
	Let $X \in \Rmn$ with $n \geq m$. If $X$ is $\tp{k}$ with $k \leq m$, then 
	\begin{enumerate}[a)]
		\item $\vari{u} \leq k-1 $ implies $\vari{Xu} \leq \min \{\rk(X)-1,\vari{u}\}$ 	 \label{eq:vardim}
		\item $\vari{Xu} = \vari{x}$ implies that the first non-zero element in $Xu$ has the same sign as the first non-zero element in $u$. \label{item:tp_k_order}
	\end{enumerate}
	The converse also holds if $X$ has full column rank. 
\end{prop}
If we disregard the order of sign changes in $Xu$, i.e., $X$ is simply assumed to be $\sr{k}$, then (\ref{prop:SR}) also remains true if (\ref{item:tp_k_order}) is dropped. 

The reader will notice that the number of $k$ minors of $X$ is combinatorial. For our purposes, fortunately, it will be sufficient to check the sign of consecutive minors to verify $k$-positivity \cite{fekete1912uber,fallat2017total}.

	

\begin{prop}\label{prop:con_minor_Hankel_Toep}
	Let $X \in \Rnn$ and $k \leq n$. 
	\begin{enumerate}[i.]
		\item Hankel $X$ is $\tp{k}$ if and only if all consecutive $j$-minors of $X$ are nonnegative for $1 \leq j \leq k$. 
		\item If $X$ is Toeplitz, lower triangular and such that all consecutive $j$-minors of $X_{1:n,1:j}$ are strictly positive for $1 \leq j \leq k-1$ and all consecutive $k$-minors of $X_{1:n,1:k}$ are nonnegative, then $X$ is $\tp{k}$.
	\end{enumerate} 
\end{prop}
Note that the difference between Hankel and Toeplitz matrices esteems from the fact that strictly $\tp{k}$ Hankel matrices lie densely within the set of $\tp{k}$ Hankel matrices \cite{fallat2017total}. 


 



\subsection{Variation-diminishing operators}





In virtue of Proposition~\ref{prop:op_seq}, we extend Definition~\ref{def:sc} to $\Toep{g}$ and $\Hank{g}$ as follows.
\begin{defn}
	$\Toep{g}$ and $\Hank{g}$ are $\sr{k}$ and $\tp{k}$ if the representation matrices of $\Toep{g}^n$ and $\Hank{g}^n$, respectively, are $\sr{k}$ and $\tp{k}$ for all $n \geq 1$. In particular, for $k=\infty$, we refer to them as \emph{totally} sign-regular and positive. Analogously, we call the system $G(z)$ Hankel and Toeplitz $\sr{k}$ and $\tp{k}$.
\end{defn}

The following elementary properties are then inherited from the properties of the finite dimensional compound matrix as reviewed in the Appendix of \cite{grussler2020variation}.
\begin{lem}\label{prop:close}
	Let $\{g_i\}_{i \in \mathds{N}} \subset \linf^{\mathds{N}}$ with $g^\opts = \lim_{i\to\infty} g_i \in \linf^{\mathds{N}}.$
	\begin{enumerate}
		\item Nestedness: $\Toep{g_1}$ is $\sr{k}$ if and only if $\Toep{g_1}$ is $\sr{j}$ for all $1 \leq j \leq k$. The same applies to $\Hank{g_1}$.
		\item Serial interconnection: If $\Toep{g_1}$ and $\Toep{g_2}$ are $\sr{k}$, then $\Toep{g_1 \ast g_2} = \Toep{g_1} \Toep{g_2}$ is $\sr{k}$. 
		\item Parallel interconnection: If $\Hank{g_1}$ and $\Hank{g_2}$ are $\tp{k}$, then $\Hank{g_1 + g_2} = \Hank{g_1}+ \Hank{g_2}$ is $\tp{k}$. 
		\item Closedness: If $\Toep{g_i}$ is $\sr{k}$ for all $i \in \mathds{N}$, then $\Toep{g^\opts}$ is $\sr{k}$. The same applies to $\Hank{g_i}$ and $\Hank{g^\opts}$. 
		\item Multiplication Toeplitz: If $G_1(z)$ is a first order system with $g_1 \in \NF$ and $\Toep{g_2}$ is $\tp{k}$, then $\Toep{g_1 g_2}$ is $\tp{k}$.
	\end{enumerate}
\end{lem}
The analogue of Proposition \ref{prop:SR} for Toeplitz and Hankel operators is then as follows \cite{karlin1968total}:
\begin{prop}\label{prop:sr_inf}
	Let $g \in \lint$ and $\Hank{g}$ be $\sr{k}$ with $k \geq 1$. Then,
	\begin{equation}
	\forall u \in \linf: \ \vari{u} \leq k-1 \ \Rightarrow \ \vari{\Hank{g} u} \leq \vari{u}. \label{eq:vardim_inf}
	\end{equation}
	Conversely, if (\ref{eq:vardim_inf}) holds then $\Hank{g}$  is $\sr{k}$. The same proposition holds for $\Toep{g}$.%
\end{prop}
Proposition~\ref{prop:sr_inf} is generally valid for pairs $g$ and $u$ as long as $\Hank{g} u \in \linf$, e.g., $g \in \linf$ and $u \in \lint$. %



In the sequel, we will verify sign-regularity only by inspecting consecutive minors, that is the determinant of the following matrices:
\begin{equation*}%
T_g(t,k) := \begin{pmatrix}
g(t) & g(t-1) & \dots & g(t-k+1)\\
g(t+1) & g(t) & \dots & g(t-j)\\
\vdots & \vdots & \ddots   & \vdots \\
g(t+k-1)   & g(t+k-2) & \dots & g(t)\\
\end{pmatrix}
\end{equation*}
and
\begin{equation*}%
H_g(t,k) := \begin{pmatrix}
g(t) & g(t+1) & \dots & g(t+k-1)\\
g(t+1) & g(t+2) & \dots & g(t+k)\\
\vdots & \vdots & \ddots   & \vdots \\
g(t+k-1)   & g(t+j) & \dots & g(t-2(k-1))\\
\end{pmatrix},
\end{equation*}
respectively. With a realization $(A,b,c)$, it holds then that
\begin{equation}
H_g(t,j) = \mathcal{O}_j A^{t-1}\mathcal{C}_j \label{eq:Hankel_mat_real}
\end{equation}
for the extended controllability and observability matrices
\begin{subequations}
	\begin{align}
	\mathcal{C}_j &:= \begin{pmatrix}
	b & Ab & \dots & A^{j-1} b
	\end{pmatrix}\\
	\mathcal{O}_j &:= \begin{pmatrix}
	c^\transp & A^\transp c^\transp & \dots & {A^\transp}^{j-1} c^\transp
	\end{pmatrix}^\transp.
	\end{align}
\end{subequations}






 

 


















==> sec_vardim_revised.tex <==


\subsection{Variation diminishing matrices}
The theory of variation diminishing matrices is a classical subject, e.g., extensively studied in the monograph \cite{karlin1968total}. Variation diminishing properties of a matrix $X \in \Rmn$ are studied via the sign-definiteness of the compound matrices $C_r(X)$, whose $(i,j)-th$ entry is defined by $\det(X_{(I,J)})$, where $I$ is the $i-th$ and $J$ is the $j-th$ element in $\mathcal{I}_{n,r}$ and $\mathcal{I}_{m,r}$, respectively. 
For example, if $X \in \mathbb{R}^{3 \times 3}$, then $C_{[2]}(X)$ reads
\begin{align*}
\begin{pmatrix}
\det(X_{\{1,2 \},\{1,2 \}}) & \det(X_{\{1,2 \},\{1,3\}}) & \det(X_{\{1,2 \},\{2,3\}})\\
\det(X_{\{1,3 \},\{1,2 \}}) & \det(X_{\{1,3 \},\{1,3\}}) & \det(X_{\{1,3 \},\{2,3\}})\\
\det(X_{\{2,3 \},\{1,2 \}}) & \det(X_{\{2,3 \},\{1,3\}}) & \det(X_{\{2,3 \},\{2,3\}})\\
\end{pmatrix}.
\end{align*}
made of all $r$-minors. 
By the \emph{extended Cauchy-Binet formula} \cite{karlin1968total} with $X \in \mathbb{R}^{n \times p}$ and $Y \in \mathbb{R}^{p \times m}$
\begin{equation}
\det((XY)_{I,J}) = \sum_{K \in \mathcal{I}_{p,r}} \det(X_{I,K}) \det(Y_{K,J}), \label{eq:CB}
\end{equation}
where $I \in \mathcal{I}_{n,r}$, $J \in \mathcal{J}_{m,r}$ and $r \leq p$, it easy to verify the following well-known properties \cite[Chapter~6]{fiedler2008special}. 
\begin{lem}\label{lem:compound_mat}
	Let $X \in \mathbb{R}^{n \times p}$, $Y \in \mathbb{R}^{p \times m}$ and $r \in \mathds{Z}_{\geq 1}$.
	\begin{enumerate}[i)]
		\item $C_{[r]}(XY) = C_{[r]}(X)C_{[r]}(Y)$.
		\item $\sigma(C_{[r]}(X)) = \{\prod_{i \in I} \lambda_i(X): I \in \mathcal{I}_{n,r} \}$.
		\item If $X \succeq 0$, then $C_{[r]}(X) \succeq 0$.
	\end{enumerate} 
\end{lem}

\begin{defn}[Sign-consistency and -regularity]
\label{def:sc}
	A matrix is called \emph{ $k$-sign consistent}  if all its  minors of order $k$ have the same sign. The property is {\it strict} if none of those minors is zero. 
The same matrix  is called \emph{(strictly) $k$-sign regular}, if it is (strictly) $j$-sign consistent for all $1 \leq j \leq k$. It is called {\emph (strictly)  $k$-positive} if the sign of minors is the same for all $1 \leq j \leq k$.
\end{defn}

The relationship between the variation diminishing property and the above definitions is provided by combining the results \cite[Theorem~5.1.1.4, Theorem~5.1.1.5,Theorem~5.2.2.4,]{karlin1968total} as follows.
\begin{prop} \label{prop:SR}
	Let $X \in \Rmn$ with $n \geq m$. If $X$ is $\tp{k}$ with $k \leq m$, then 
	\begin{enumerate}[a)]
		\item $\vari{u} \leq k-1 $ implies $\vari{Xu} \leq \min \{\rk(X)-1,\vari{u}\}$ 	 \label{eq:vardim}
		\item $\vari{Xu} = \vari{x}$ implies that the first non-zero element in $Xu$ has the same sign as the first non-zero element in $u$. \label{item:tp_k_order}
	\end{enumerate}
	The converse also holds if $X$ has full column rank. 
\end{prop}
If we disregard the order of sign changes in $Xu$, i.e., $X$ is simply assumed to be $\sr{k}$, then (\ref{prop:SR}) also remains true if (\ref{item:tp_k_order}) is dropped. 

The reader will notice that the number of $k$ minors of $X$ is combinatorial. For our purposes, fortunately, it will be sufficient to check the sign of consecutive minors to verify $k$-positivity \cite{fekete1912uber,fallat2017total}.

	

\begin{prop}\label{prop:con_minor_Hankel_Toep}
	Let $X \in \Rnn$ and $k \leq n$. 
		If $X$ is Toeplitz, lower triangular and such that all consecutive $j$-minors of $X_{1:n,1:j}$ are strictly positive for $1 \leq j \leq k-1$ and all consecutive $k$-minors of $X_{1:n,1:k}$ are nonnegative, then $X$ is $\tp{k}$.
\end{prop}

The consequence of Proposition \ref{prop:con_minor_Hankel_Toep} is that variation diminishing properties of causal LTI systems  only requires to inspect consecutive minors, that is the determinant of the following matrices:
\begin{equation*}%
T_g(t,k) := \begin{pmatrix}
g(t) & g(t-1) & \dots & g(t-k+1)\\
g(t+1) & g(t) & \dots & g(t-j)\\
\vdots & \vdots & \ddots   & \vdots \\
g(t+k-1)   & g(t+k-2) & \dots & g(t)\\
\end{pmatrix}
\end{equation*}



 



\subsection{Variation-diminishing operators}





In virtue of Proposition~\ref{prop:op_seq}, we extend Definition~\ref{def:sc} to $\Toep{g}$   as follows.
\begin{defn}
	$\Toep{g}$  is  $\sr{k}$ and $\tp{k}$ if the representation matrices of $\Toep{g}^n$  are $\sr{k}$ and $\tp{k}$ for all $n \geq 1$. In particular, for $k=\infty$, we refer to them as \emph{totally} sign-regular and positive. Analogously, we call the system $G(z)$ $\tp{k}$.
\end{defn}

The following elementary properties are then inherited from the properties of the finite dimensional compound matrix as reviewed in the Appendix of \cite{grussler2020variation}.
\begin{lem}\label{prop:close}
	Let $\{g_i\}_{i \in \mathds{N}} \subset \linf^{\mathds{N}}$ with $g^\opts = \lim_{i\to\infty} g_i \in \linf^{\mathds{N}}.$
	\begin{enumerate}
		\item Nestedness: $\Toep{g_1}$ is $\sr{k}$ if and only if $\Toep{g_1}$ is $\sr{j}$ for all $1 \leq j \leq k$.  
		\item Serial interconnection: If $\Toep{g_1}$ and $\Toep{g_2}$ are $\sr{k}$, then $\Toep{g_1 \ast g_2} = \Toep{g_1} \Toep{g_2}$ is $\sr{k}$.  
		\item Closedness: If $\Toep{g_i}$ is $\sr{k}$ for all $i \in \mathds{N}$, then $\Toep{g^\opts}$ is $\sr{k}$.  
		\item Multiplication : If $G_1(z)$ is a first order system with $g_1 \in \NF$ and $\Toep{g_2}$ is $\tp{k}$, then $\Toep{g_1 g_2}$ is $\tp{k}$.
	\end{enumerate}
\end{lem}
The analogue of Proposition \ref{prop:SR} for the Toeplitz operator is  as follows \cite{karlin1968total}:
\begin{prop}\label{prop:sr_inf}
	Let $g \in \lint$ and $\Toep{g}$ be $\sr{k}$ with $k \geq 1$. Then,
	\begin{equation}
	\forall u \in \linf: \ \vari{u} \leq k-1 \ \Rightarrow \ \vari{\Toep{g} u} \leq \vari{u}. \label{eq:vardim_inf}
	\end{equation}
	Conversely, if (\ref{eq:vardim_inf}) holds then $\Toep{g}$  is $\sr{k}$. %
\end{prop}
Proposition~\ref{prop:sr_inf} is generally valid for pairs $g$ and $u$ as long as $\Toep{g} u \in \linf$, e.g., $g \in \linf$ and $u \in \lint$. %



\subsection{Variation-diminishing Hankel operators}

The variation diminishing properties of the Toeplitz operator are closely related to the variation diminishing properties of the Hankel operator. 
This is because the analogue of $T_g(t,k)$ for the Hankel operator is the matrix
\begin{equation*}%
H_g(t,k) := \begin{pmatrix}
g(t) & g(t+1) & \dots & g(t+k-1)\\
g(t+1) & g(t+2) & \dots & g(t+k)\\
\vdots & \vdots & \ddots   & \vdots \\
g(t+k-1)   & g(t+j) & \dots & g(t-2(k-1))\\
\end{pmatrix},
\end{equation*}

Note that if $t-j\geq 0$, then $T_g(t,j)$ can be transformed into $H_g(t-j+1,j)$ through reversion of the  column/row order, i.e., $\det(T_g(t,j)) = \xi(j)\det(H_g(t-j+1,j))$ where 
	\begin{equation}
	\xi(j) := \begin{cases}
	1 & \text{if } j \mod 4 \leq 1\\
	-1 & \text{else}
	\end{cases}.
	\end{equation}
	
It will be sometimes  convenient to study the properties of   $\det(T_g(t,j))$ via the properties of $det(H_g(t-j+1,j))$. In particular, we will take advantage of the classical formula
\begin{equation}
H_g(t,j) = \mathcal{O}_j A^{t-1}\mathcal{C}_j \label{eq:Hankel_mat_real}
\end{equation}
for the extended controllability and observability matrices
\begin{subequations}
	\begin{align}
	\mathcal{C}_j &:= \begin{pmatrix}
	b & Ab & \dots & A^{j-1} b
	\end{pmatrix}\\
	\mathcal{O}_j &:= \begin{pmatrix}
	c^\transp & A^\transp c^\transp & \dots & {A^\transp}^{j-1} c^\transp
	\end{pmatrix}^\transp.
	\end{align}
\end{subequations}
that applies to any state-space realization $(A,b,c)$.


	





 

 

















